Stochastic Leadtimes and Order Crossover: A Damped Response to a Weighted Inventory Position

Inventory control with stochastic leadtimes is a classical problem of inventory theory. When orders can cross it remains a challenging one: the base-stock policy need not be optimal, and the optimal policy is still unknown. We offer two insights about crossover. Outstanding orders may arrive late, so they should count for less than their size. An order placed later may arrive early, so the order placed now should not close the whole gap to its target. These two discounts give the policy its structure, a damped response to a weighted inventory position. We propose two ways to set them, and neither needs a search. The first is a closed form that uses the leadtime distribution alone: an outstanding order counts with the probability that it arrives no later than a new one. The second takes one further step and uses the costs: an outstanding order counts by how often it is missing when the stock is about to run out. Both policies perform very well against the optimal cost, lower bounds that need no dynamic program, and the existing policies. On 405 instances they are 0.48% and 0.11% above the optimal cost on average, against 2.04% for the base-stock policy.

==> sections/gen/numbers.tex <==
\makeatletter
\@namedef{nv@lr.all.n}{405}
\@namedef{nv@lr.all.bs.med}{0.38}
\@namedef{nv@lr.all.bs.mean}{2.04}
\@namedef{nv@lr.all.bs.max}{30.31}
\@namedef{nv@lr.all.paper.med}{0.13}
\@namedef{nv@lr.all.paper.mean}{0.48}
\@namedef{nv@lr.all.paper.max}{5.07}
\@namedef{nv@lr.all.lin.mean}{0.07}
\@namedef{nv@lr.all.lin.max}{1.12}
\@namedef{nv@lr.all.lbu.mean}{2.54}
\@namedef{nv@lr.all.lbu.max}{13.75}
\@namedef{nv@lr.all.lbk.mean}{0.76}
\@namedef{nv@lr.all.lbk.max}{8.86}
\@namedef{nv@lr.all.p2.med}{0.03}
\@namedef{nv@lr.all.p2.mean}{0.11}
\@namedef{nv@lr.all.p2.max}{1.84}
\@namedef{nv@lr.all.p2.belowp1}{326}
\@namedef{nv@lr.all.p2.abovep1}{14}
\@namedef{nv@lr.all.p2.excessp1}{0.049}
\@namedef{nv@lr.skew.bs.mean}{3.30}
\@namedef{nv@lr.skew.bs.max}{30.31}
\@namedef{nv@lr.skew.paper.mean}{0.79}
\@namedef{nv@lr.skew.paper.max}{5.07}
\@namedef{nv@lr.skew.lin.mean}{0.10}
\@namedef{nv@lr.skew.lin.max}{1.12}
\@namedef{nv@lr.skew.lbu.mean}{3.17}
\@namedef{nv@lr.skew.lbu.max}{13.75}
\@namedef{nv@lr.skew.lbk.mean}{1.18}
\@namedef{nv@lr.skew.lbk.max}{8.86}
\@namedef{nv@lr.skew.p2.mean}{0.17}
\@namedef{nv@lr.skew.p2.max}{1.84}
\@namedef{nv@lr.mid.bs.mean}{0.46}
\@namedef{nv@lr.mid.bs.max}{3.17}
\@namedef{nv@lr.mid.paper.mean}{0.10}
\@namedef{nv@lr.mid.paper.max}{1.18}
\@namedef{nv@lr.mid.lin.mean}{0.03}
\@namedef{nv@lr.mid.lin.max}{0.27}
\@namedef{nv@lr.mid.lbu.mean}{1.75}
\@namedef{nv@lr.mid.lbu.max}{9.14}
\@namedef{nv@lr.mid.lbk.mean}{0.23}
\@namedef{nv@lr.mid.lbk.max}{3.14}
\@namedef{nv@lr.mid.p2.mean}{0.04}
\@namedef{nv@lr.mid.p2.max}{0.30}
\@namedef{nv@lr.b1.bs.mean}{2.90}
\@namedef{nv@lr.b1.bs.max}{30.31}
\@namedef{nv@lr.b1.paper.mean}{0.24}
\@namedef{nv@lr.b1.paper.max}{2.89}
\@namedef{nv@lr.b1.lin.mean}{0.04}
\@namedef{nv@lr.b1.lin.max}{0.30}
\@namedef{nv@lr.b1.lbu.mean}{3.58}
\@namedef{nv@lr.b1.lbu.max}{13.75}
\@namedef{nv@lr.b1.lbk.mean}{1.15}
\@namedef{nv@lr.b1.lbk.max}{8.86}
\@namedef{nv@lr.b1.p2.mean}{0.12}
\@namedef{nv@lr.b1.p2.max}{1.84}
\@namedef{nv@lr.b2.bs.mean}{2.50}
\@namedef{nv@lr.b2.bs.max}{30.22}
\@namedef{nv@lr.b2.paper.mean}{0.26}
\@namedef{nv@lr.b2.paper.max}{2.35}
\@namedef{nv@lr.b2.lin.mean}{0.04}
\@namedef{nv@lr.b2.lin.max}{0.24}
\@namedef{nv@lr.b2.lbu.mean}{3.16}
\@namedef{nv@lr.b2.lbu.max}{12.30}
\@namedef{nv@lr.b2.lbk.mean}{0.95}
\@namedef{nv@lr.b2.lbk.max}{8.35}
\@namedef{nv@lr.b2.p2.mean}{0.08}
\@namedef{nv@lr.b2.p2.max}{0.48}
\@namedef{nv@lr.b4.bs.mean}{2.01}
\@namedef{nv@lr.b4.bs.max}{21.57}
\@namedef{nv@lr.b4.paper.mean}{0.46}
\@namedef{nv@lr.b4.paper.max}{5.07}
\@namedef{nv@lr.b4.lin.mean}{0.06}
\@namedef{nv@lr.b4.lin.max}{0.57}
\@namedef{nv@lr.b4.lbu.mean}{2.61}
\@namedef{nv@lr.b4.lbu.max}{12.45}
\@namedef{nv@lr.b4.lbk.mean}{0.75}
\@namedef{nv@lr.b4.lbk.max}{8.34}
\@namedef{nv@lr.b4.p2.mean}{0.11}
\@namedef{nv@lr.b4.p2.max}{1.16}
\@namedef{nv@lr.b9.bs.mean}{1.52}
\@namedef{nv@lr.b9.bs.max}{14.75}
\@namedef{nv@lr.b9.paper.mean}{0.64}
\@namedef{nv@lr.b9.paper.max}{2.76}
\@namedef{nv@lr.b9.lin.mean}{0.09}
\@namedef{nv@lr.b9.lin.max}{0.70}
\@namedef{nv@lr.b9.lbu.mean}{1.94}
\@namedef{nv@lr.b9.lbu.max}{9.50}
\@namedef{nv@lr.b9.lbk.mean}{0.54}
\@namedef{nv@lr.b9.lbk.max}{4.89}
\@namedef{nv@lr.b9.p2.mean}{0.12}
\@namedef{nv@lr.b9.p2.max}{0.83}
\@namedef{nv@lr.b19.n}{81}
\@namedef{nv@lr.b19.bs.mean}{1.25}
\@namedef{nv@lr.b19.bs.max}{13.03}
\@namedef{nv@lr.b19.paper.mean}{0.81}
\@namedef{nv@lr.b19.paper.max}{3.70}
\@namedef{nv@lr.b19.lin.mean}{0.10}
\@namedef{nv@lr.b19.lin.max}{1.12}
\@namedef{nv@lr.b19.lbu.mean}{1.43}
\@namedef{nv@lr.b19.lbu.max}{7.89}
\@namedef{nv@lr.b19.lbk.mean}{0.41}
\@namedef{nv@lr.b19.lbk.max}{5.56}
\@namedef{nv@lr.b19.p2.mean}{0.13}
\@namedef{nv@lr.b19.p2.max}{1.30}
\@namedef{nv@lr.mu5.bs.mean}{1.95}
\@namedef{nv@lr.mu5.bs.max}{14.37}
\@namedef{nv@lr.mu5.paper.mean}{0.34}
\@namedef{nv@lr.mu5.paper.max}{2.51}
\@namedef{nv@lr.mu5.lin.mean}{0.06}
\@namedef{nv@lr.mu5.lin.max}{0.62}
\@namedef{nv@lr.mu5.lbu.mean}{2.92}
\@namedef{nv@lr.mu5.lbu.max}{12.47}
\@namedef{nv@lr.mu5.lbk.mean}{0.73}
\@namedef{nv@lr.mu5.lbk.max}{5.86}
\@namedef{nv@lr.mu5.p2.mean}{0.10}
\@namedef{nv@lr.mu5.p2.max}{0.74}
\@namedef{nv@lr.mu10.bs.mean}{2.03}
\@namedef{nv@lr.mu10.bs.max}{21.09}
\@namedef{nv@lr.mu10.paper.mean}{0.47}
\@namedef{nv@lr.mu10.paper.max}{2.80}
\@namedef{nv@lr.mu10.lin.mean}{0.07}
\@namedef{nv@lr.mu10.lin.max}{0.88}
\@namedef{nv@lr.mu10.lbu.mean}{2.54}
\@namedef{nv@lr.mu10.lbu.max}{13.25}
\@namedef{nv@lr.mu10.lbk.mean}{0.76}
\@namedef{nv@lr.mu10.lbk.max}{7.24}
\@namedef{nv@lr.mu10.p2.mean}{0.10}
\@namedef{nv@lr.mu10.p2.max}{1.18}
\@namedef{nv@lr.mu20.bs.mean}{2.12}
\@namedef{nv@lr.mu20.bs.max}{30.31}
\@namedef{nv@lr.mu20.paper.mean}{0.63}
\@namedef{nv@lr.mu20.paper.max}{5.07}
\@namedef{nv@lr.mu20.lin.mean}{0.07}
\@namedef{nv@lr.mu20.lin.max}{1.12}
\@namedef{nv@lr.mu20.lbu.mean}{2.17}
\@namedef{nv@lr.mu20.lbu.max}{13.75}
\@namedef{nv@lr.mu20.lbk.mean}{0.79}
\@namedef{nv@lr.mu20.lbk.max}{8.86}
\@namedef{nv@lr.mu20.p2.mean}{0.13}
\@namedef{nv@lr.mu20.p2.max}{1.84}
\@namedef{nv@lr.r2skew.bs.mean}{0.37}
\@namedef{nv@lr.r2skew.bs.max}{1.29}
\@namedef{nv@lr.r2skew.paper.mean}{0.14}
\@namedef{nv@lr.r2skew.paper.max}{0.66}
\@namedef{nv@lr.r2skew.lin.mean}{0.02}
\@namedef{nv@lr.r2skew.lin.max}{0.08}
\@namedef{nv@lr.r2skew.lbu.mean}{0.83}
\@namedef{nv@lr.r2skew.lbu.max}{2.51}
\@namedef{nv@lr.r2skew.lbk.mean}{0.13}
\@namedef{nv@lr.r2skew.lbk.max}{0.51}
\@namedef{nv@lr.r2skew.p2.mean}{0.03}
\@namedef{nv@lr.r2skew.p2.max}{0.13}
\@namedef{nv@lr.r2mid.bs.mean}{0.09}
\@namedef{nv@lr.r2mid.bs.max}{0.54}
\@namedef{nv@lr.r2mid.paper.mean}{0.02}
\@namedef{nv@lr.r2mid.paper.max}{0.15}
\@namedef{nv@lr.r2mid.lin.mean}{0.00}
\@namedef{nv@lr.r2mid.lin.max}{0.03}
\@namedef{nv@lr.r2mid.lbu.mean}{0.41}
\@namedef{nv@lr.r2mid.lbu.max}{1.66}
\@namedef{nv@lr.r2mid.lbk.mean}{0.02}
\@namedef{nv@lr.r2mid.lbk.max}{0.19}
\@namedef{nv@lr.r2mid.p2.mean}{0.01}
\@namedef{nv@lr.r2mid.p2.max}{0.09}
\@namedef{nv@lr.r3q9.bs.mean}{8.65}
\@namedef{nv@lr.r3q9.paper.mean}{1.17}
\@namedef{nv@lr.r3q9.p2.mean}{0.18}
\@namedef{nv@lr.r3skew.bs.mean}{3.11}
\@namedef{nv@lr.r3skew.bs.max}{15.40}
\@namedef{nv@lr.r3skew.paper.mean}{0.89}
\@namedef{nv@lr.r3skew.paper.max}{2.95}
\@namedef{nv@lr.r3skew.lin.mean}{0.09}
\@namedef{nv@lr.r3skew.lin.max}{0.34}
\@namedef{nv@lr.r3skew.lbu.mean}{3.08}
\@namedef{nv@lr.r3skew.lbu.max}{7.28}
\@namedef{nv@lr.r3skew.lbk.mean}{0.82}
\@namedef{nv@lr.r3skew.lbk.max}{2.72}
\@namedef{nv@lr.r3skew.p2.mean}{0.14}
\@namedef{nv@lr.r3skew.p2.max}{0.48}
\@namedef{nv@lr.r3mid.bs.mean}{0.43}
\@namedef{nv@lr.r3mid.bs.max}{1.74}
\@namedef{nv@lr.r3mid.paper.mean}{0.11}
\@namedef{nv@lr.r3mid.paper.max}{0.86}
\@namedef{nv@lr.r3mid.lin.mean}{0.03}
\@namedef{nv@lr.r3mid.lin.max}{0.13}
\@namedef{nv@lr.r3mid.lbu.mean}{1.67}
\@namedef{nv@lr.r3mid.lbu.max}{5.43}
\@namedef{nv@lr.r3mid.lbk.mean}{0.13}
\@namedef{nv@lr.r3mid.lbk.max}{0.68}
\@namedef{nv@lr.r3mid.p2.mean}{0.04}
\@namedef{nv@lr.r3mid.p2.max}{0.23}
\@namedef{nv@lr.r4skew.bs.mean}{6.41}
\@namedef{nv@lr.r4skew.bs.max}{30.31}
\@namedef{nv@lr.r4skew.paper.mean}{1.33}
\@namedef{nv@lr.r4skew.paper.max}{5.07}
\@namedef{nv@lr.r4skew.lin.mean}{0.19}
\@namedef{nv@lr.r4skew.lin.max}{1.12}
\@namedef{nv@lr.r4skew.lbu.mean}{5.62}
\@namedef{nv@lr.r4skew.lbu.max}{13.75}
\@namedef{nv@lr.r4skew.lbk.mean}{2.59}
\@namedef{nv@lr.r4skew.lbk.max}{8.86}
\@namedef{nv@lr.r4skew.p2.mean}{0.34}
\@namedef{nv@lr.r4skew.p2.max}{1.84}
\@namedef{nv@lr.r4mid.bs.mean}{0.86}
\@namedef{nv@lr.r4mid.bs.max}{3.17}
\@namedef{nv@lr.r4mid.paper.mean}{0.16}
\@namedef{nv@lr.r4mid.paper.max}{1.18}
\@namedef{nv@lr.r4mid.lin.mean}{0.05}
\@namedef{nv@lr.r4mid.lin.max}{0.27}
\@namedef{nv@lr.r4mid.lbu.mean}{3.18}
\@namedef{nv@lr.r4mid.lbu.max}{9.14}
\@namedef{nv@lr.r4mid.lbk.mean}{0.54}
\@namedef{nv@lr.r4mid.lbk.max}{3.14}
\@namedef{nv@lr.r4mid.p2.mean}{0.06}
\@namedef{nv@lr.r4mid.p2.max}{0.30}
\@namedef{nv@pipe.all.atbound}{8}
\@namedef{nv@bed.n}{405}
\@namedef{nv@net.exact.n}{162}
\@namedef{nv@net.exact.diff.max}{0.002}
\@namedef{nv@simcal.n}{135}
\@namedef{nv@simcal.pout.max}{0.04}
\@namedef{nv@simcal.wi.mean}{0.005}
\@namedef{nv@simcal.wi.max}{0.21}
\@namedef{nv@simcal.lin.max}{0.01}
\@namedef{nv@pipesim.n}{45}
\@namedef{nv@pipesim.mean}{0.012}
\@namedef{nv@pipesim.max}{0.033}
\@namedef{nv@net.r2.n}{135}
\@namedef{nv@net.r2.gamma1}{132}
\@namedef{nv@net.r2.equal}{134}
\@namedef{nv@net.r2.se}{0.0017}
\@namedef{nv@net.r3.se}{0.0058}
\@namedef{nv@net.r3.exact}{27}
\@namedef{nv@net.r4.se}{0.0106}
\@namedef{nv@lr.all.above.t}{104}
\@namedef{nv@lr.b19.above.t}{42}
\@namedef{nv@lr.all.wi.above.t}{235}
\@namedef{nv@lr.all.wi.below.t}{150}
\@namedef{nv@lr.all.wi.abovep2.t}{308}
\@namedef{nv@lr.all.wi.belowp2.t}{29}
\@namedef{nv@lmin.r3.base_stock.1.mean}{1.92}
\@namedef{nv@lmin.r3.base_stock.2.mean}{0.48}
\@namedef{nv@lmin.r4.base_stock.2.mean}{1.59}
\@namedef{nv@lmin.r4.base_stock.3.mean}{0.70}
\@namedef{nv@lmin.all.base_stock.0.mean}{7.22}
\@namedef{nv@lmin.all.complete.0.mean}{2.19}
\@namedef{nv@lmin.all.p2.0.mean}{0.48}
\@namedef{nv@lmin.all.p2.abovep1.0}{33}
\@namedef{nv@lmin.all.p2.abovep1.0.mid}{29}
\@namedef{nv@lmin.all.p2.abovep1.0.b12}{26}
\@namedef{nv@lmin.all.p2.abovep1.0.max}{0.99}
\@namedef{nv@lmin.all.p2.abovebs.0}{6}
\@namedef{nv@lmin.all.p2.abovebs.0.max}{0.13}
\@namedef{nv@zero.all.lin.max}{0.50}
\@namedef{nv@zero.n}{36}
\@namedef{nv@zero.opt.diff}{0.02}
\@namedef{nv@zero.p2.belowall}{26}
\@namedef{nv@top.lr.balance.pow}{-9}
\@namedef{nv@box.rel.pow}{-10}
\@namedef{nv@edge.lmin1p.pow}{-5}
\@namedef{nv@edge.lmin0.p2.mant}{1.2}
\@namedef{nv@edge.lmin0.p2.pow}{-4}
\@namedef{nv@wi.w0.min}{0.97}
\@namedef{nv@p2.negw.1}{5}
\@namedef{nv@p2.negw.1.n}{405}
\@namedef{nv@p2.negw.1.min}{-0.015}
\@namedef{nv@p2.negw.0}{1}
\@namedef{nv@p2.negw.0.min}{-0.0001}
\@namedef{nv@p2.def.n}{2430}
\@namedef{nv@p2.def.radius}{0.78}
\@namedef{nv@p2.def.raw}{1.13}
\@namedef{nv@p2.def.rounds}{46}
\@namedef{nv@p2.def.ricits}{112}
\@namedef{nv@quad.bed.thmin}{0.002}
\@namedef{nv@quad.ex.th1}{0.193}
\@namedef{nv@quad.ex.th2}{0.747}
\@namedef{nv@quad.ex.th3}{-0.007}
\@namedef{nv@quad.ex.th4}{0.093}
\@namedef{nv@quad.ex.th5}{0.257}
\@namedef{nv@quad.ex.kappa}{0.929}
\@namedef{nv@p2.proj.n}{113}
\@namedef{nv@p2.proj.0}{78}
\@namedef{nv@p2.proj.1}{30}
\@namedef{nv@p2.proj.2}{5}
\@namedef{nv@p2.exist.n}{810}
\@namedef{nv@p2.exist.margin3}{0.119}
\@namedef{nv@p2.scan.n}{1251}
\@namedef{nv@p2.scan.multi}{3}
\@namedef{nv@chain.r3.n}{90}
\@namedef{nv@chain.r3.age1.viol}{29}
\@namedef{nv@chain.r4.n}{45}
\@namedef{nv@chain.r4.age1.viol}{16}
\@namedef{nv@chain.r4.age2.viol}{17}
\@namedef{nv@chain.all.age1.mass}{0.64}
\@namedef{nv@long.r2.bs.5.mean}{0.55}
\@namedef{nv@long.r2.bs.5.max}{1.68}
\@namedef{nv@long.r2.bs.20.mean}{0.24}
\@namedef{nv@long.r2.bs.20.max}{0.55}
\@namedef{nv@long.r2.bs.100.mean}{0.06}
\@namedef{nv@long.r2.bs.100.max}{0.12}
\@namedef{nv@long.r2.bs.500.mean}{0.01}
\@namedef{nv@long.r2.bs.500.max}{0.02}
\@namedef{nv@long.r2.bs.lim.mean}{6.4}
\@namedef{nv@long.r2.bs.lim.max}{12.5}
\@namedef{nv@long.r2.p1.5.mean}{0.44}
\@namedef{nv@long.r2.p1.5.max}{1.18}
\@namedef{nv@long.r2.p1.20.mean}{0.19}
\@namedef{nv@long.r2.p1.20.max}{0.42}
\@namedef{nv@long.r2.p1.100.mean}{0.05}
\@namedef{nv@long.r2.p1.100.max}{0.10}
\@namedef{nv@long.r2.p1.500.mean}{0.01}
\@namedef{nv@long.r2.p1.500.max}{0.02}
\@namedef{nv@long.r2.p1.lim.mean}{5.6}
\@namedef{nv@long.r2.p1.lim.max}{10.3}
\@namedef{nv@long.r2.p2.5.mean}{0.42}
\@namedef{nv@long.r2.p2.5.max}{1.17}
\@namedef{nv@long.r2.p2.20.mean}{0.19}
\@namedef{nv@long.r2.p2.20.max}{0.42}
\@namedef{nv@long.r2.p2.100.mean}{0.05}
\@namedef{nv@long.r2.p2.100.max}{0.10}
\@namedef{nv@long.r2.p2.500.mean}{0.01}
\@namedef{nv@long.r2.p2.500.max}{0.02}
\@namedef{nv@long.r2.p2.lim.mean}{5.5}
\@namedef{nv@long.r2.p2.lim.max}{10.1}
\@namedef{nv@long.dp.r2.bs.20.mean}{0.052}
\@namedef{nv@long.dp.r2.bs.20.max}{0.188}
\@namedef{nv@long.dp.r2.p1.20.mean}{0.004}
\@namedef{nv@long.dp.r2.p1.20.max}{0.034}
\@namedef{nv@long.dp.r2.p2.20.mean}{0.001}
\@namedef{nv@long.dp.r2.p2.20.max}{0.005}
\@namedef{nv@long.dp.r2.bs.100.mean}{0.011}
\@namedef{nv@long.dp.r2.bs.100.max}{0.039}
\@namedef{nv@long.dp.r2.p1.100.mean}{0.000}
\@namedef{nv@long.dp.r2.p1.100.max}{0.003}
\@namedef{nv@long.dp.r2.p2.100.mean}{0.000}
\@namedef{nv@long.dp.r2.p2.100.max}{0.000}
\@namedef{nv@long.r3.bs.5.mean}{1.36}
\@namedef{nv@long.r3.bs.5.max}{3.39}
\@namedef{nv@long.r3.bs.20.mean}{0.64}
\@namedef{nv@long.r3.bs.20.max}{1.30}
\@namedef{nv@long.r3.bs.100.mean}{0.17}
\@namedef{nv@long.r3.bs.100.max}{0.30}
\@namedef{nv@long.r3.bs.500.mean}{0.04}
\@namedef{nv@long.r3.bs.500.max}{0.06}
\@namedef{nv@long.r3.bs.lim.mean}{18.2}
\@namedef{nv@long.r3.bs.lim.max}{31.2}
\@namedef{nv@long.r3.p1.5.mean}{1.04}
\@namedef{nv@long.r3.p1.5.max}{2.32}
\@namedef{nv@long.r3.p1.20.mean}{0.49}
\@namedef{nv@long.r3.p1.20.max}{0.93}
\@namedef{nv@long.r3.p1.100.mean}{0.13}
\@namedef{nv@long.r3.p1.100.max}{0.22}
\@namedef{nv@long.r3.p1.500.mean}{0.03}
\@namedef{nv@long.r3.p1.500.max}{0.05}
\@namedef{nv@long.r3.p1.lim.mean}{14.3}
\@namedef{nv@long.r3.p1.lim.max}{23.1}
\@namedef{nv@long.r3.p2.5.mean}{1.01}
\@namedef{nv@long.r3.p2.5.max}{2.30}
\@namedef{nv@long.r3.p2.20.mean}{0.48}
\@namedef{nv@long.r3.p2.20.max}{0.92}
\@namedef{nv@long.r3.p2.100.mean}{0.13}
\@namedef{nv@long.r3.p2.100.max}{0.22}
\@namedef{nv@long.r3.p2.500.mean}{0.03}
\@namedef{nv@long.r3.p2.500.max}{0.05}
\@namedef{nv@long.r3.p2.lim.mean}{14.3}
\@namedef{nv@long.r3.p2.lim.max}{22.8}
\@namedef{nv@long.dp.r3.bs.20.mean}{0.154}
\@namedef{nv@long.dp.r3.bs.20.max}{0.413}
\@namedef{nv@long.dp.r3.p1.20.mean}{0.010}
\@namedef{nv@long.dp.r3.p1.20.max}{0.067}
\@namedef{nv@long.dp.r3.p2.20.mean}{0.001}
\@namedef{nv@long.dp.r3.p2.20.max}{0.008}
\@namedef{nv@long.dp.r3.bs.100.mean}{0.041}
\@namedef{nv@long.dp.r3.bs.100.max}{0.096}
\@namedef{nv@long.dp.r3.p1.100.mean}{0.001}
\@namedef{nv@long.dp.r3.p1.100.max}{0.006}
\@namedef{nv@long.dp.r3.p2.100.mean}{0.000}
\@namedef{nv@long.dp.r3.p2.100.max}{0.000}
\@namedef{nv@long.r4.bs.5.mean}{2.13}
\@namedef{nv@long.r4.bs.5.max}{5.05}
\@namedef{nv@long.r4.bs.20.mean}{1.05}
\@namedef{nv@long.r4.bs.20.max}{2.08}
\@namedef{nv@long.r4.bs.100.mean}{0.29}
\@namedef{nv@long.r4.bs.100.max}{0.52}
\@namedef{nv@long.r4.bs.500.mean}{0.06}
\@namedef{nv@long.r4.bs.500.max}{0.11}
\@namedef{nv@long.r4.bs.lim.mean}{31.8}
\@namedef{nv@long.r4.bs.lim.max}{53.1}
\@namedef{nv@long.r4.p1.5.mean}{1.59}
\@namedef{nv@long.r4.p1.5.max}{3.71}
\@namedef{nv@long.r4.p1.20.mean}{0.78}
\@namedef{nv@long.r4.p1.20.max}{1.53}
\@namedef{nv@long.r4.p1.100.mean}{0.21}
\@namedef{nv@long.r4.p1.100.max}{0.37}
\@namedef{nv@long.r4.p1.500.mean}{0.05}
\@namedef{nv@long.r4.p1.500.max}{0.08}
\@namedef{nv@long.r4.p1.lim.mean}{23.7}
\@namedef{nv@long.r4.p1.lim.max}{39.7}
\@namedef{nv@long.r4.p2.5.mean}{1.54}
\@namedef{nv@long.r4.p2.5.max}{3.68}
\@namedef{nv@long.r4.p2.20.mean}{0.76}
\@namedef{nv@long.r4.p2.20.max}{1.52}
\@namedef{nv@long.r4.p2.100.mean}{0.21}
\@namedef{nv@long.r4.p2.100.max}{0.37}
\@namedef{nv@long.r4.p2.500.mean}{0.05}
\@namedef{nv@long.r4.p2.500.max}{0.08}
\@namedef{nv@long.r4.p2.lim.mean}{23.6}
\@namedef{nv@long.r4.p2.lim.max}{39.5}
\@namedef{nv@long.dp.r4.bs.20.mean}{0.283}
\@namedef{nv@long.dp.r4.bs.20.max}{0.714}
\@namedef{nv@long.dp.r4.p1.20.mean}{0.015}
\@namedef{nv@long.dp.r4.p1.20.max}{0.091}
\@namedef{nv@long.dp.r4.p2.20.mean}{0.002}
\@namedef{nv@long.dp.r4.p2.20.max}{0.014}
\@namedef{nv@long.dp.r4.bs.100.mean}{0.078}
\@namedef{nv@long.dp.r4.bs.100.max}{0.176}
\@namedef{nv@long.dp.r4.p1.100.mean}{0.002}
\@namedef{nv@long.dp.r4.p1.100.max}{0.008}
\@namedef{nv@long.dp.r4.p2.100.mean}{0.000}
\@namedef{nv@long.dp.r4.p2.100.max}{0.001}
\@namedef{nv@long.p2conv.5.max}{0.26}
\@namedef{nv@long.p2conv.500.max}{0.040}
\makeatother

